CLASP: Constrained Latent Shape Projection for Refining Object Shape from Robot Contact

Robots need both visual and contact sensing to effectively estimate the state of their environment. Camera RGBD data provides rich information of the objects surrounding the robot, and shape priors can help correct noise and fill in gaps and occluded regions. However, when the robot senses unexpected contact, the estimate should be updated to explain the contact. To address this need, we propose CLASP: Constrained Latent Shape Projection. This approach consists of a shape completion network that generates a prior from RGBD data and a procedure to generate shapes consistent with both the network prior and robot contact observations. We find CLASP consistently decreases the Chamfer Distance between the predicted and ground truth scenes, while other approaches do not benefit from contact information.

==> sections/conclusion.tex <==
% !TEX root = ../main.tex


\section{Conclusion}

We demonstrated a method for estimating shape completions initialized with purely RGBD visual data, then updated from observations of a robot arm moving through unknown regions and sensing contact.
We stored the belief of the scene as a particle filter of latent vectors from a shape completions network and used \ourmethod{} to enforce shape consistency with the robot observations.
Most importantly, we showed that CLASP improves the estimate of object shape using these contact observations.
Our results further showed that \ourmethod{} performs better than ablations of \ourmethod{} and alternative methods. 
We hope CLASP will be used within a larger robotics framework where reasoning over environment uncertainty based on shape priors aids in accomplishing larger goals.
% \asnote{I feel like I want a little bit more here at the end to tie up your work with a nice big bow. Maybe something big-picture or application based, future work?}

==> sections/evaluation.tex <==
% !TEX root = ../main.tex

\subsection{Quantifying Plausibility} \label{sec:evaluation}








==> sections/zz_old_problem_formulation.tex <==
% !TEX root = ../main.tex

\section{Problem Formulation} \label{sec:problem}

\bsnote{This problem formulation has good roots for a future paper (ICRA?), but does has more complexity and less learning than I really want for this CoRL paper}

Consider a robot $\robot$ operating in a world $\world$ of static (immovable)  objects $\{\object_1, \object_2, ...\} \in \Objects$.
The robot can move in C-space in this world, accumulating cost $\cost = (Distance\ moved)$.
The objects induce C-space obstacles.
The objects also induce a goal set $\goalset$ from a goal generator function $G(\Objects)\rightarrow \goalset$.
Each goal $\goal \in \goalset$ is in $\cspace \times \action$. The goal action $\action_g$ has some (large) associated cost.
% The goal set is determined from a goal generator 
Our task is complected by moving the configuration any goal $\goal \subset \goalset$ and execute that goal's action $\action_g$.
Our objective is to complete the task with minimal cost.


(If the objects of this world are known, this problem can be approximately solved with standard Motion Planning to first move to a configuration, then executing the goal action).

Consider the situation where the objects are not known exactly, but are instead observed initially using a depth camera, and further observed through contact (as described in the BTP paper) as the robot moves around $\cspace$.

Assumptions
\begin{itemize}
    \item Objects are ``similar" to objects seen before (so a shape completer might capture them)
    \item Segmenter capable of segmenting objects
\end{itemize}

Other details
\begin{itemize}
\item The robot is equipped with a camera and contact sensing (as described in BTP paper).
\end{itemize}



